Adopting Road-Weather Open Data in Route Recommendation Engine

Digitraffic, Finland's open road data interface, provides access to nationwide road sensors with more than 2,300 real-time attributes from 1,814 stations. However, efficiently utilizing such a versatile data API for a practical application requires a deeper understanding of the data qualities, preprocessing phases, and machine learning tools. This paper discusses the challenges of large-scale road weather and traffic data. We go through the road-weather-related attributes from DigiTraffic as a practical example of processes required to work with such a dataset. In addition, we provide a methodology for efficient data utilization for the target application, a personalized road recommendation engine based on a simple routing application. We validate our solution based on real-world data, showing we can efficiently identify and recommend personalized routes for three different driver profiles.

==> dataset-old.tex <==
\section{Digitraffic: Road-Weather Data} \label{roaddata}
\input{datatable}

\begin{comment}
\begin{figure}[htp]
    \centering
    \includegraphics[width=0.5\textwidth]{pictures/factors.drawio.png}
    \caption{Dynamic factors affecting the traversability of a road segment}
    \label{fig:galaxy}
\end{figure}
\end{comment}

% Kameroita on koko maassa 761, niiltä saa kuvia 2077 eri suunnasta,
% current weatherista saa irti 148 eri attribuuttia (529 sääasemalta)
% liikennemääristä saa 103 attribuuttia (520 mittauspaikalta)
% sääennusteen nyt ehkä laskisin yheksi kokonaisuudeksi koska loppupelissä sen tarkotus on antaa vaan luokitus onko ajosää hyvää/huonoa/erittäin huonoa. Toki jos lasketaan kaikki eri aikamääreiden ennusteet niin saahaan nykyhetki, 2h, 4h, 6h, 12h -> 5
% liikennetiedotteita nuo 4
% muuttuvat tieliikennemerkit, periaatteessa 2, koska varoitusnäytöt ja nopeusnäytöt
% kunnossapitovahtauksesta 2, sijainnit ja tehdyt työt
% Mitä nuo sit yhteensä tekee, 2341 tiedonmurua?

\color{black}
Digitraffic is an open data service provided by Fintraffic, a traffic management entity owned by the Finnish Ministry of Transport and Communications. It provides traffic data in real time through open APIs. The data offered through the road API includes images from road weather cameras, current weather measurements, road weather forecasts, traffic measurements and alerts, data displayed on variable message signs, road maintenance tracking, and measurements from pedestrian counting sites. Additionally, metadata about the measurement sites and the data itself is updated twice a day and is retrievable through the API \cite{digitrafficLiikennetilanne}.  % should this be a footnote rather than a reference?
%[TO-DO] add pedestrian counting to the table
In addition to road traffic data, Digitraffic also provides open data about railway and maritime traffic, which will not be discussed further in this article, as well as data from pedestrian counting sites, which was likewise ignored.

% A similar service can be found in New South Wales, Australia, called Live Traffic NSW, which provides information about incidents and adverse weather, rest areas, car parks, as well as Google produced traffic flow status and live traffic camera images. The service also comes with a route calculator, but this tool does not appear to take any of the above mentioned into consideration with the route planning, instead producing a list of "hazards" along the route for the user to note about the suggested route.
% https://www.livetraffic.com/

Our goal was to use the road traffic data to enrich route planning. To do this, we first investigated the full extent of the data available through the road traffic API, after which we moved on to defining weight vectors for a road network graph based on the open data from Digitraffic.

As of July 2024, there are 533 road weather stations, 520 traffic measurement sites, and 761 camera locations in Finland. These measurement stations collect the majority of the data available through the API, with the exception of traffic messages, variable message signs, and road maintenance vehicle locations

\subsection{Road Weather Cameras}
Of the 761 camera locations, one has been temporarily removed, leaving us with active 760 sites. Each site can have anywhere between 1 and 7 "presets", which in this context means the different directions where the camera is aimed. The most common number of presets per location is three: one in each direction of traffic and one that is aimed at the road surface itself. Pictures are updated every 10 minutes, and it is possible to retrieve all pictures taken within the past 24 hours. While camera footage could be used for various purposes as was discussed in section \ref{relwo_cameras}, including road surface state monitoring, this information can also be retrieved through the weather API. That being said, in future iterations utilising road weather camera images in addition to data from weather stations should be considered, as there are cameras in many locations without weather stations. This would help retrieve accurate data from a wider geographical area, in particular areas where there are no weather stations. 

\subsection{Road Weather Stations} \label{weatherstationdata}
According to the meta as of a July 2024, 529 weather stations are actively gathering data, while four have temporarily been removed. Interestingly enough, 58 of these \textit{road} weather stations are actually located at airport runways. The data produced by these stations will not be used for the weight vectors, as the state on the surface of a runway cannot be directly linked to that on ordinary roads even if they are located nearby. Excluding these stations leaves us with 471 active road weather stations. 
Vast majority of these stations are labelled as one of two station types: ROSA or RWS\_200. These coincide with the names of two types of road weather stations distributed by Vaisala, ROSA and RWS200, of which ROSA has been discontinued \cite{vaisalaUpgradeROSA}. As the stations are commercial products (that further utilise other commercial products), information about them is limited and documentation at times scarce.  While some information from Vaisala is available about the sensors and the values they produce (such as in the station product catalogue \cite{RWS200ProductCatalog}), this information is limited and at times hard to link back to the attributes present in the Digitraffic API. This makes understanding the API output sometimes a challenge. Attributes carrying categorical information such as weather conditions and road surface states are particularly problematic, as despite these classes being listed with their names in the specific sensor documentation, the values returned for the attributes are numerical instead of strings. In cases where no distinction about the sensor used is made in the meta data in addition to no value descriptions, it is effectively impossible to know which states the attribute is trying to communicate.

The road weather stations employ a wide variety of sensors to gather data about their surroundings. The data from sensors can be fetched either through a JSON API, or with an MQTT WebSocket. The sensor attributes are given identifiers between 1 and 226, although meta data can only be fetched for 148 sensors as it appears the rest are not currently used. % fetch with /api/weather/v1/sensors.
The meta includes identifiers, names, units, accuracy, and value descriptions for sensors. The level of detail in the documentation varies greatly between sensors – in some cases the descriptions are very in-depth, for example by providing explanations for enumerate values, while others are missing basic things like units. Additionally, some sensors seem to measure the same thing, for example there are four near identical attributes for road surface temperature %TIE_1, TIE_2, TIE_3, TIE_4 (id:3, 5, 101, 111)
It is likely that different sensors measure temperature on different lanes, however this is not explicitly stated anywhere. It could also be that the multiple sensors guarantee reliability, which would be very important as the temperature of the road surface is a vital piece of information for many applications of road weather data.

In preparation for vector weight definitions, the attributes were thematically categorised into four groups based on how they affect road traffic. These categories were road surface conditions, visibility, other environmental factors (e.g. extreme temperatures and high winds), and those that do not influence driving conditions enough for us to consider at this time, or that are too ambiguous to categorise. By combining the previously discussed duplicate variables into one attribute, we were left with 86 attributes to sort. 
The next sections detail the eventual classification of the attributes, and their roles in weight vector definition.

% [TO-DO]: REMEMBER TO MENTION THE WHOLE FOUR ATTRIBUTES PER VALUE BUT ONLY ABOUT 1/10 STATIONS ACTUALLY USE THAT MANY! Also check is there a relation between the number of sensors used & the number of lanes per road; we know that ouluntulli uses 2 of most, raahe only 1! but this isn't like a hard set rule...
\subsubsection{Road Surface}
The condition of the road surface is one of the most important factors affecting driving.
These attributes make a great deal of difference in how easily a car can be handled, and how quickly it can be stopped in an emergency.

There are several attributes that offer classifications of the conditions on the surface of the road. These attributes are perhaps the most expressive ones when it comes to information conveyed by a single attribute. Their usefulness is further enforced by the fact that they are among the most common attributes actively updated by weather stations.
One attribute classifies the conditions as:
\begin{itemize}
    \item Dry % -> 0 [1]
    \item Moist % -> 0,125[2]
    \item Wet % -> 0,25 [3]
    \item Most likely moist and salty % -> 0,375 [8]
    \item Wet and salted (salting agent has been spread on the road) % -> 0,5 [4]
    \item Frost % -> 0.625 [5]
    \item Ice % -> 0.75 [7]
    \item Snow % -> 0.875 [6]
    \item Slush % -> 1 [9]
\end{itemize}
% 27	KELI_1
% 28	KELI_2
% 105	KELI_3
% 115	KELI_4
Slush is the most dangerous surface state as it is linked to a significantly higher accident risk than most other states, including dry, moist, frosty, and even icey roads \cite{malin2019accident}. Therefore slush was considered the worst one of the possible surface states, and given the weight of 1. Dry road surface was likened to the absence of environmental hindrances, therefore it received the weight of 0. Moist was rated at 0.125, wet at 0.25. Their salted counterparts were ranked slightly higher, with moist and salty at 0.375 and wet and salted at 0.5. The presence of salting agents implies a higher risk for the formation of ice and slush. 
Malin et al \cite{malin2019accident} found a higher risk for accidents to be associated with snowy rather than icey roads, perhaps due to the fact the snow fall can often come on suddenly, and be linked to snow fall, while some roads might be icey throughout winter, and therefore represent a continuous state rather than abnormal conditions. A frosty road is also associated with a higher relative risk of accidents than moist roads, but lower than snowy or icey roads. Therefore, frosty roads were assigned the weight of 0.625, icey 0.75 and snowy 0.875.

Ranking the road surface conditions is difficult, even from a perspective of accident minimisation, as different combinations of surface and precipitation conditions contribute to very different relative risks. For example, a slushy road with no precipitation can be related to a higher risk of accidents than an icey one, however with heavy precipitation, an icey road becomes more than twice as accident prone as a slushy road with similar precipitation \cite{malin2019accident}. Specific combination of factors can be extremely dangerous even if separately these two factors have a much smaller effect on driving conditions. An example of such a case is light snow fall combined with temperatures below -7°C, as the two factors together make for very slippery roads that cannot be salted \cite{FMIconditions}. 
With this is mind, this ranking of road surface states on their own is an approximation and should be taken with a grain of salt.

There are also two other attributes that describe the road surface conditions, however these attributes provide numerical values with no value descriptions, and as such we are unable to decipher the condition communicated by these attributes. Therefore the above is the only surface condition attribute one we will consider for the weight vectors.
% 167	TIENPINNAN_TILA_1 -> discard
% 168	TIENPINNAN_TILA_2 -> discard
% 169	TIENPINNAN_TILA_3 -> discard
% 170	TIENPINNAN_TILA_4 -> discard
% 174	OPTISEN_ANTURIN_KELI1 -> discard
% 184	OPTISEN_ANTURIN_KELI2 -> discard

The weather stations measure the depth of moisture in general, or more specifically water, snow, and ice on the road, all provided via their own attributes in millimetres. There are at least three sensors that can provide this data or a portion of it: the DSC optical sensor, DRS511 embedded sensor, and a water level and snow depth sensor by Campbell Scientific \cite{RWS200ProductCatalog}. This makes determining the value ranges a challenge. The maximum values of the DSC sensor appear to be the smallest at 2.00 mm, and the DSR511 can detect water levels up to 7mm, while the Campbell Scientific SR50A does not give a definitive limit, but can output values up to 9999 mm. 
% MOISTURE:
% 50	KOSTEUDEN_MÄÄRÄ_1; near all stations
% 51	KOSTEUDEN_MÄÄRÄ_2
% 198	KOSTEUDEN_MÄÄRÄ_3
% 199	KOSTEUDEN_MÄÄRÄ_4
% ==> get an average of these present; 0mm --> 0; max --> 1 
% WATER:
% 177	VEDEN_MÄÄRÄ1 // dsc: 0.00-2.00 mm; => discard
% 187	VEDEN_MÄÄRÄ2 // dsc: 0.00-2.00 mm => discard
% SNOW:
% 178	LUMEN_MÄÄRÄ1 // DSC; half of stations; => discard
% 188	LUMEN_MÄÄRÄ2 // DSC => discard
% 94	LUMEN_SYVYYS => 0 -> 0, 10 -> 1
% ICE:
% 179	JÄÄN_MÄÄRÄ1 // dsc: 0.00-2.00 mm => discard
% 189	JÄÄN_MÄÄRÄ2 // dsc: 0.00-2.00 mm => discard
Additionally, a thicker layer often means more challenging driving conditions, though not always. More water lessens friction, as does a thick layer of snow - enough fresh snow on the road surface might prevent the wheels of the vehicle from touching the solid surface of the road at all.
Ice is a more complicated form of moisture, as it does lessen friction, and thick layers of ice can be linked to deep ruts that make steering a challenge, however a thin layer of slippery ice on the road surface can arguably be even more dangerous as it can be harder to detect.
Regardless, as the attribute conveying the unspecified moisture level is a separate and far more common attribute than the more specific ones (with the exception of snow depth, which is equally common), we had to work under the assumption that a thicker layer denotes further deteriorated conditions. The maximum layer thickness proved equally challenging, as we only knew that this value was produced by a "surface sensor", but not which one – as the DRS511 had a lower maximum than the Campbell sensor, we elected to follow that one. This set the maximum weight of 1 at 7mm, with 0mm being weighted at 0 and 3.5mm at 0.5.
The only specific moisture attribute that was commonly available was the snow depth. This is presumably provided by a different station, as instead of millimetres, the value is given in centimetres, according to the meta. It is likely that this value is measured by the SR50A sensor. As the SR50A documentation we could find %https://s.campbellsci.com/documents/cr/manuals/sr50a.pdf
did not contain explicit value ranges, except for when the value is reported in millimetres for which the maximum value is 9999 mm. However, even in Finland, nearly 10 metres of snow on the road surface is not likely. On the other hand, snowfall of 10 to 15 cm overnight is certainly not unheard of, and it can definitely cause difficulties for drivers. Therefore, we, perhaps somewhat arbitrarily, chose 10 cm as our maximum value for the snow depth, with 0 cm being the logical minimum value.

As was indicated friction of the road surface is important factor that greatly affects the driving experience. The API provides this data as a value between 0.09 – 0.82µ, 
% 176	KITKA1
% 181	KITKA1_LUKU  -> disgard; the same as the first
% 186	KITKA2
% 191	KITKA2_LUKU -> disgard; the same as the first
which greatly complements our understanding of the current state of the road surface conditions provided by the condition categories. Less friction can be make driving unsafe, therefore should the friction value be 0.09, the weight of the friction factor will be 1. Friction of 0.82µ will lead to weight of 0. The values in between will be scaled evenly, e.g. the friction value of 0.455µ will result in a weight of 0.5.

In winter conditions, friction can be improved by using salting agents on the road surface. The Digitraffic API provides data on both the amount of agents present on the road surface, as well as the concentration of said agents. The amounts are given as grams per square metre, while the concentration is given as grams per litre.
% 52	SUOLAN_MÄÄRÄ_1 => discard
% 53	SUOLAN_MÄÄRÄ_2 => discard
% 200	SUOLAN_MÄÄRÄ_3 => discard
% 201	SUOLAN_MÄÄRÄ_4 => discard
% 54	SUOLAN_VÄKEVYYS_1 => discard
% 55	SUOLAN_VÄKEVYYS_2 => discard
% 202	SUOLAN_VÄKEVYYS_3 => discard
% 203	SUOLAN_VÄKEVYYS_4 => discard
However, excessive amounts of road salt do not guarantee the best possible driving conditions. Road salt is notorious for corroding cars, its effectiveness worsens when the temperature drops below -6 degrees Celsius, and in a worst case scenario, excessive salting in sub-optimal conditions can lead to the formation of even more slippery ice, should the melted water freeze again \cite{vaylavirastoTalvikunnossapito}. It can also promote the formation of slush, which Malin et al \cite{malin2019accident} found to be among the most detrimental factors to road safety. All that being said, using the amount and concentration of salt on the road to assess the driving conditions is a very tricky task, and often heavily dependant on the driver's preferences. The friction and surface conditions as a result of the use of salt are generalisable, therefore they were used instead of the salt attributes for the weight creation.

Malin et al also found that when the temperature of the road surface drops from +2°C to -2°C, the risk of accidents increases rapidly, after which the risk slowly decreases, but remains elevated compared to temperatures above freezing \cite{malin2019accident}. The API provides the road surface temperature at an accuracy of one decimal. A single station can have up to five road temperature readings, and some stations can even provide the temperate 30 cm below ground. 
% 3	TIE_1
% 5	TIE_2
% 101	TIE_3
% 111	TIE_4
% 172	TIEN_LÄMPÖTILA_DST-ANT -> disgard
% 12	RUNKO_1 -> discard
While extremely high road surface temperature can soften the road surface and cause other issues, in the Finnish context this extreme is negligibly rare and therefore largely omitted from our work. Instead, our focus was on the temperatures identified by Malin et al \cite{malin2019accident} as the most dangerous ones. The relative accident risk peaks at -2°C, therefore we will consider this our maximum value and assign the weight of 1 to it. The minimum values for the high and low are not symmetrical to reflect the relative risks. On the positive end of the temperature scale, the risk only begins to elevate at +2°C. To include a small safety buffer, we set the minimum weight of 0 at the temperature of +5°C and higher. The other minimum was set at -20°C to account for the slow decline of the risk index with the falling temperatures as presented in Figure 2 of Malin et al \cite{malin2019accident}, with the values in between scaling proportionally.

The Digitraffic API includes many other road temperature related attributes, that focus more so on the accumulation of potential moisture on the road rather than the temperature itself. The weather stations monitor the dew point of the road, as well as the freezing and frost points. While these limit values are important, for route planning they are only meaningful when compared to the current temperature. 
% 10	JÄÄTYMISPISTE_1; use together with road temp; see scale from dew point.
% 11	JÄÄTYMISPISTE_2
% 104	JÄÄTYMISPISTE_3
% 114	JÄÄTYMISPISTE_4
% 126	KUURAPISTE => discard
% 56	TURVALLISUUSLÄMPÖ_1 => discard
% 57	TURVALLISUUSLÄMPÖ_2 => discard
% 204	TURVALLISUUSLÄMPÖ_3 => discard
% 205	TURVALLISUUSLÄMPÖ_4 => discard
Luckily, this has been taken somewhat into consideration, as the API also offers attributes that provide the difference between the limit value and the current temperature of the road and air for both dew and frost points. In the context of the road surface, we used the ones that did the comparison to the road surface temperature rather than air. While the temperature is above freezing, the values of the dew point and frost point are usually the same, but once the temperature drops below freezing, they start to differ. As the attributes conveying the dew point are commonly available, when the temperature is above freezing, we elected to use it exclusively for weight creation. Once below freezing, we used the frost point attributes, with the exception of weather stations that did not carry this attribute, in which case we only used the dew point attributes. 
The choice of using the dew point when the temperature is above freezing and the frost point while it is below is based on a recommendation from Vaisala documentation %https://www.vaisala.com/sites/default/files/documents/VIM-GLO-EN-HUM-Dew_point_frost_point_selection_%20B212716EN-A.pdf
% 49	KASTEPISTE_ERO_TIE 0=>1, 5=>0
% 226	KASTEPISTE_ERO_TIE2
% 127	KUURAPISTE_ERO_TIE => discard

As notable differences in conditions only begin to emerge once the difference between the dew or frost point and the current temperature becomes very small, for the most part if there is a difference, the value should not affect route planning. If there is no difference, or the difference is negative, the weight is set to 1. To account for measuring errors and to add a small safety buffer as conditions might change rather rapidly, the weight of 0 is set when the difference is 5°C or more. The values in between 0°C and 5°C are scaled proportionally so that the weight of 0.5 corresponds to the temperature difference of 2.5°C.

The freezing point does not have a similar temperature difference attribute as the dew and frost point do. Instead, we had to calculate the difference ourselves. The same values were used for the weight generation as for the dew and frost point differences. Additionally, there are two freezing points, one representing the "true" freezing point while the other one has an additional safety buffer added to it. As the true freezing point is more common, we elected to use it over the "safety point", as the 5°C gradually increasing weight as the freezing point approaches, provides a buffer of its own.

\subsubsection{Visibility}
It goes without saying that poor visibility increases the risk of accidents, as drivers struggle to observe their surroundings. The Digitraffic API provides visibility as both metres and kilometres, produced by two different kinds of sensors, of which the remote DSC sensor is far more rare. The DSC and the PWD12 sensors can detect distances up to 2 km while the PWD22 sensor can detect them up to 20 km \cite{RWS200ProductCatalog}. These two distinct max values make determining the weight scale a challenge, however based on data queries made on clear days, it would seem that the majority of stations have equipped the PWD22 sensor and can in fact detect distances up to 20 km. The PWD values capped at 2000 m seem to appear only at 13 stations along road 1 in southern Finland, one station in Keuruu, and 4 stations located at airports. Therefore, we will ignore these outliers and consider 20 km as the general maximum detectable value.
% 160	NÄKYVYYS_DSC_1 => 10–2000 m with DSC211
% 161	NÄKYVYYS_DSC_2
% 26	NÄKYVYYS_KM (PWD sensor) 0-2 or 20 depending on the station..?
% 58	NÄKYVYYS_M (PWD sensor) 0-2000 or 20000 depending on the station
% PWD sensors are A LOT more common, DSC sensor values are only available at <= 30 stations.
% most stations have both km and m measures but some (19/532) are even still capped at 2000. Of which the only ones in Northern ostrobothnia are at the airport so we don't care? Not at this point. 
Visibility can be considered good when it is more than 10 kilometres, moderate when it is 4-10 kilometres, poor at 1-4 kilometres, and very poor when it is under 1 kilometre. Visibility below one kilometre indicated the presence of fog \cite{ilmatieteenlaitosNakyvyys}. 
% so use this as a scale? 0-999m => 1-0.91, 1000-3999 => 0.9-0.61, 4000-10000m => 0.60-0.00.
Based on this, the weight of the visibility factor was set to 0 if the detected visibility was 10 km or more, and 1 should the visibility have fallen to 0. The values in between were scaled proportionally.

Fog can form when the dew point falls below the temperature of air. The API contains attributes for the dew point itself as well as the difference between the dew point and air temperature. For assessing driving conditions, the difference attribute gives direct value as a smaller difference would mean a higher risk for fog formation. The frost point was considered in temperatures below freezing, similarly to what was discussed above with the road surface weights. The value range considered here is the same as above, i.e. the weight of 0 for a difference in temperatures that is 5°C or more and 1 for differences of 0°C and less.
% 9	    KASTEPISTE; useless alone => discard
% 73    KASTEPISTE_ERO_ILMA; closer to zero -> higher cost.
% 128	KUURAPISTE_ERO_ILMA
The relative humidity of air is also closely related to this. Fog tends to form in conditions when the relative humidity is at least 90\%. Therefore, the closer the percentage from the API is to 100, the closer the cost is to 1.
% 21    ILMAN_KOSTEUS; 0% -> 0, 100% -> 1.


Precipitation of various types is another major factor affecting visibility and with, the driving conditions. The type of precipitation as well as its intensity play a key role in determining the affect it has on driving conditions. Rain, sleet, and snow are each associated with a higher risk of accidents than the previous, and this risk also increases with the intensity of the precipitation \cite{malin2019accident}. The Digitraffic API has multiple attributes available detailing the precipitations conditions on the road. The system is able to determine if the current precipitation is drizzle, rain, snow, wet sleet, regular sleet, hail, ice crystals, snow grains, snow pellets, or freezing drizzle or freezing rain. In some cases when the precipitation is very weak, it might not be possible to determine the type. 
% 25	SATEEN_OLOMUOTO_PWDXX
Both Tobin et al. \cite{tobin2021adverseweather}
and Malin et al. \cite{malin2019accident} found snow more perilous than rain. In Malin et al, sleet (rain/snow mixed) was found to be more dangerous than rain, but less dangerous than snow. Freezing drizzle and freezing rain were not ranked with the other precipitation types, but the associated relative risk associated with them would fall in between sleet and snow. In comparison, in Tobin et al snow is associated with a higher risk than rain, but a lower risk than freezing rain. Sleet (ice pellets) is considered more dangerous than rain, but defining a more specific spot for it in the hierarchy was not possible. Any type of precipitation is linked to a higher relative risk than dry weather. 
% dry, rain, sleet, freezing drizzle / rain, snow
% dry, rain, snow, freezing rain; ice pellets is something else
Our ranking of the precipitation types was done based mostly on these two papers, as most other papers focus on the intensity of precipitation, or use even more crude categorisations of precipitation, such as only considering regular rain versus snow.
% e.g. Andrey, J., Mills, B., Leahy, M. et al. Weather as a Chronic Hazard for Road Transportation in Canadian Cities. Natural Hazards 28, 319–343 (2003). https://doi.org/10.1023/A:1022934225431
Dry weather was considered the optimal conditions, therefore it was assigned the weight of 0.0. Precipitation that was too weak to determine its type was considered the second most optimal, followed by the various types of rain ranked based on their intensities. Neither paper distinguished between wet and regular sleet (rain/snow mix), but we reasoned that since wet sleet is closer to regular rain, it would be considered less dangerous than regular sleet that could be considered more similar to snow. Hail was excluded from analysis in Tobin et al.\cite{tobin2021adverseweather}, nor could be find comparable studies that would have specified the risk associated hail. We reasoned that they should be considered more of a hindrance than sleet as hail tends to fall rapidly in large quantities, impacting visibility and potentially causing loss of traction, but less troublesome than snowfall as hailstorms are typically shorter in duration. 
Ice crystals, snow grain and snow pellets were considered sub-types of snow. The final challenge was deciding, which should be ranked more dangerous, freezing rain or snow. It is possible that geographical distance explain the difference in accident risks in a study done on Finnish data \cite{malin2019accident} and a study done on data from Kansas \cite{tobin2021adverseweather}, as the intensity and frequency of the phenomena can be vastly different. Legislative difference may also play a part, for example winter tyres are mandatory in Finland but are not necessarily so in the US. As a kind of compromise, we ranked freezing drizzle below snow in danger, while freezing rain was placed above snow. Table \ref{tab:precipitation_table} presents the final ranking of conditions, and their weights.

\begin{table}[ht]
    \centering
    \begin{tabular}{| c | c |}
    \hline
        Condition & Weight \\
        \hline
        Dry weather & 0.0 \\
        Weak precipitation, type cannot be determined & 0.111 \\
        Drizzle & 0.222 \\
        Rain & 0.333 \\
        Wet sleet & 0.444 \\
        Sleet & 0.556 \\
        Hail & 0.667 \\
        Freezing drizzle & 0.778 \\
        Snow & 0.889 \\
        Freezing rain & 1.0 \\ 
        \hline 
    \end{tabular}
    \caption{Ranking of precipitation conditions and the weights associated with each condition from 0.0 to 1.0.}
    \label{tab:precipitation_table}
\end{table}

This ranking should be further evaluated in the future with the help of statistical analysis, especially regarding the precipitation types that have not yet been considered in literature. In the future, it should also be considered whether specific precipitation types should be weighted differently based on other variables, such as road surface condition and temperature.
% 7.0: Pouta, dry weather -> 0
% 8.0: Hyvin heikko sade, olomuotoa ei voida päätellä, -> 1
% 9.0: Tihku, drizzle -> 2
% 10.0 Vesisade, rain -> 3
% 11.0: Lumisade, snow -> 8
% 12.0: Märkä räntä, ? -> 4
% 13.0: Räntä, sleet -> 5
% 14.0 Rakeita, hail -> 6
% 15.0: Jääkiteitä, ice crystals -> snow -> 8
% 16.0: Lumijyväsiä, snow grain -> snow -> 8
% 17.0: Lumirakeita, snow pellet/graupel -> snow -> 8
% 18.0: Jäätävä tihku, freezing drizzle -> 7
% 19.0: Jäätävä sade, freezing rain -> 9

There are stations where this attribute is not available. In such cases, or when the detailed precipitation type is not available, we elected to use another attribute, which classifies precipitation as either rain or sleet/snow. To emulate the weights from the previous attribute, if the reported precipitation type is sleet/snow, the weight will be set to 0.722, which is the average of the weights for sleet and snow as we cannot know which type is in question at any given time. The same attribute also classifies precipitation based on intensity to either weak, moderate, or abundant. Again, to best emulate the weights determined with the more precise attribute, weak rain was likened to drizzle and given the weight 0.222, while both moderate and abundant rain were given the weight of 0.333.

% 22 SADE   => discard
The intensity is also provided in millilitres.
% 23 SADE_INTENSITEETTI => 0 -> 0, 10mm/h -> 1 
The Swagger documentation of the API provides a classification for rain intensities in millilitres into similar intensity categories with slightly different names of light rain, rain, and heavy rain. Rain is considered heavy when the intensity is more than 7.6 mm per hour. Rainfall of 7 mm/h or more is considered intense rain by the FMI. 
%https://www.ilmatieteenlaitos.fi/sade 
To account for differences even with more intense rainfalls, we set the value to be weighted at the maximum weight of 1 to be 10.0 mm/h. Unsurprisingly, the minimum weight of 0 was set to the value of 0.0 mm/h, with the values in between scaling proportionally.

Additionally, the system records the sum of daily precipitation. These values is not too relevant to us, as their main importance to us would be to assess how much water could be on the surface of the road, for which purpose we already have another attribute measuring this directly.
%24	SADESUMMA   => discard
%215 SADESUMMA_LIUKUVA_24H => discard
There are also two attributes that give the precipitation status as either a boolean value of 1 or 0, or as an enumerate status based on the overall status of the station, but these attributes will not be used. The boolean precipitation status is only available at a couple of stations (despite the meta claiming otherwise), while the enumerate one does not include any value descriptions, nor could any definitive conclusions be made based on the values of other attributes. 
% 225	SADE I/O (only available from 1/2 stations) => discard
% 48	SADE_TILA (cannot make rhyme or reason from the values) => discard



\subsubsection{Other Environmental Factors}
% [TO-DO] joku kuva missä eri environmental factorit tulee esiteltyä? Kategorisoittain; tuuli, lämpö, jne?
While the influence of visibility and road surface conditions on driving is rather obvious, other environmental factors are more easily overlooked. High winds can make steering challenging and pick up dirt that decreases visibility. They can also cause trees to fall on the road causing obstructions. Similarly, both extreme cold and heat can hinder travels. Among other consequences, cold weather can cause condensation to form in the fuel tank, causing the engine problems, while hot weather can lead to the engine overheating. 

The API offers data on the average and maximum wind speeds from the past 10 minutes, in addition to providing the average direction of the wind.
%16	KESKITUULI      => wind factor;
%17	MAKSIMITUULI    => wind factor
%18	TUULENSUUNTA    => discard
While the wind speeds can be used for weight vectors on their own, direction is different. To make it relevant for driving, one would need to know the direction in which the vehicle would be heading on the road. This would allow increasing the weight on segments experiencing cross winds, which can be particularly dangerous. However this process was deemed outside the scope of this project and therefore only the immediately usable attributes of average and maximum wind were used. Highest possible wind speed reported by the RWS200 weather station is 75 m/s \cite{RWS200ProductCatalog}. The Finnish Meteorological institute (FMI) categorises winds into seven categories based on average speeds from 0 m/s to 33 m/s and faster, which would be defined as hurricane \cite{ilmatieteenlaitosTuuli}. However, such a high wind average has never been measured in Finland %https://www.ilmatieteenlaitos.fi/tuulitilastot TODO
Winds measuring 21 m/s and faster are classified storm winds \cite{ilmatieteenlaitosTuuli}, leading up to which, The FMI issues wind warnings once the average wind speed reaches 15 m/s (in summer) or 20 m/s (in winter). %source here [TO-DO] https://www.ilmatieteenlaitos.fi/tuulivaroitukset
It is normal for gusts of wind to be 1.5 to 2 times more intense than the measured average winds. Therefore, it was justified to consider different weights for the average and maximum winds. Based on the previous, we set the maximum average wind to 21 m/s, which would be given the weight of 1, while the maximum value for maximum wind speed was set to 31.5 m/s, which is 1.5 times the maximum average speed we set. Winds of 0 m/s were set as the minimum for both.

As previously stated, extreme temperatures can have detrimental affect on driving conditions. The Digitraffic API provides multiple temperature measurements on top of the road surface temperatures discussed earlier. These include current air and ground temperature, as well as the minimum and maximum air temperatures from the past 24 hours. For now, the historical values were discarded as the focus is on the current conditions. We also ignore the ground temperature, as we believe that the temperatures from the air and the road surface are more pertinent to driving conditions.
% 1	ILMA => [1,0,1] -30, +14, +27
% 7	MAA_1 => ignore
% 8	MAA_2 => ignore
% 103	MAA_3 => ignore
% 113	MAA_4 => ignore
% 213	ILMAN_LÄMPÖTILA_24H_MIN => discard
% 214	ILMAN_LÄMPÖTILA_24H_MAX => discard
The FMI releases an alert for heat once the temperature of is predicted to reach +27°C. %https://www.ilmatieteenlaitos.fi/tietoa-helle-ja-pakkasvaroitukset 
We will consider this our max heat value and assign any vector with this value or higher the weight of one. Defining the threshold for harsh frost is more complex, as the FMI has determined different thresholds for different parts of the country. The Northern Ostrobothnia falls into the northern part of the country, which would place our other max value at -30°C. The midpoint between the values would be 0°C, and the weight could be determined by the difference between the midpoint and the current air temperature, with 0.0 degrees leading to the weight of zero, and the difference of 30 degrees to the weight of one. A more advanced approach would be to consider the heat and frost differently, as Finns generally are more accustomed to cold than heat. According to the FMI, the "optimal" temperature for Finnish people is 14°C, with rising temperatures bringing adverse consequences much faster than a drop in temperature does. 
% https://www.ilmatieteenlaitos.fi/aarilampotilojen-terveysvaikutuksia
In this case, the temperature of 14°C would be yield the cost of 0, -30°C and +27°C the cost of 1, and values in between would be weighted based on the relative distance from 14°C. For example, the temperature of 20.5°C would be assigned the weight of 0.5 as it is midway between the optimal temperature of 14°C and +27°C. The weight of 0.5 would also be assigned should the air temperature be -8°C as this is the midway between the optimal temperature and -30°C.

\subsubsection{Other Variables}
% [TO-DO] intro to this; why they were "disqualified"; this category is composed of attributes describing the status of the station, as well as weather attributes that we cannot utilise at this time for one reason or anohter.
While attributes describing the status of the station itself are certainly valuable for maintenance and fault detection purposes, this data does not enhance our understanding of the conditions on the road. The status of the station is communicated via multiple attributes, which describe present sensor faults, % ANTURIVIKA (no unit or values described; numerical code; present in data query for stations that do have issues; atm only with ROSA stations???)
statuses of specific sensors systems, including things like sensor cleanliness, 
% DSC_STAT1
% DSC_STAT2
% DSC_VASTAANOTTIMEN_PUHTAUS, 
% PWD_LÄHETTIMEN_TAKAISINSIRONNAN_MUUTOS, 
% PWD_VASTAANOTTIMEN_TAKAISINSIRONNAN_MUUTOS 
% PWD_STATUS
% PWD_TILA
% PWD_NÄK_TILA
or the overall status of the station. 
% ASEMAN_STATUS (2; "hälytys, sade, keli"), 
% ASEMAN_STATUS_OPT (2; "hälytys, keli"); should this be in the other environmental...? 
The status can communicate warnings about the conditions on the road, however these warnings tend to be rather general, for example only providing values such as OK, BEWARE, ALARM, FROST, and RAIN. 
% OPTISEN_ANTURIN_VAROITUS1 (175) and 2 (185)) 
% 29	VAROITUS_1
% 30	VAROITUS_2
% 106	VAROITUS_3
% 116	VAROITUS_4

Some attributes related to the weather conditions were excluded from feature creation. This was either due to their nature or the fact that they were only available at a handful of weather stations. For example, many attributes in the attribute meta list describe aspects of solar radiation, % AURINGON_IR_SATEILY_ALAS (144; w/m^2), 
% AURINGON_IR_SATEILY_ULOS (143; W/m^2),
% AURINGON_SATEILY_ALAS (142; W/m^2)
% AURINGON_SATEILY_ULOS (141; W/m^2)
% NETTOSÄTEILY(ANT97) (145; W/m^2)
which is a very important piece of information for developing weather forecasts, but on its own serves little purpose for route planning. Additionally, these radiation attributes are not available through the data query from any weather stations. Some stations are described in the meta as test stations for radiation measurements, therefore it is probable that this information is being gathered but not yet shared openly. 
Other sun related attributes were also excluded, namely two attributes that track the position of the sun to determine the lighting conditions. It is known that darker times of the day are more accident prone, but as we only consider route planning on a limited geographical area, and ignore the possibility of postponing travels until e.g., the morning these attributes are not useful to us at this point. This data would lend itself to some very interesting route considerations if used together with a data source that provides information about street lights present along road segments.
% 99	VALOISAA
% 98	AURINKOUP
The change rates of weather features as well as weather were excluded at this stage, as without considering the time dimension, they serve little purpose.
% ILMA_DERIVAATTA (2; C/h)
% 4	TIE_1_DERIVAATTA
% 6	TIE_2_DERIVAATTA
% 102	TIE_3_DERIVAATTA
% 112	TIE_4_DERIVAATTA
% 20	ILMANPAINE_DERIVAATTA

The attribute meta also describes several weather forecast attributes (wind speed and direction, cloudiness, precipitation intensity, type, and likelihood) that are not actually present in the data query. It is probable that these attributes refer to the data retrievable through the weather forecast API. 
% 60 TUULEN_SUUNTA_ENNUSTE
% 61 TUULEN_NOPEUS_ENNUSTE
% 62 PILVISYYS_ENNUSTE
% 63 SATEEN_OLOMUOTO_ENNUSTE
% 64 SATEEN_INTENSITEETTI_ENNUSTE
% 65 SATEEN_ESTOD_ENNUSTE
% 66 ILMAN_LÄMPÖTILA_ENNUSTE
% 67 TIEN_LÄMPÖTILA_ENNUSTE
% 68 KASTEP_LÄMPÖTILA_ENNUSTE
% 71 SADEMÄÄRÄ_1H_ENNUSTE
% 75 KASTEPISTE_ERO_TIE_ENNUSTE
We also excluded an attribute which details the current weather in WMO 4680 weather codes, as for the most part the relevant weather variables can be derived from other attributes. In the future, this could be used as a back up should other attributes not be present, or if user has specific preferences related to weather that cannot be detected via other attributes, such as thunder.
% 100 VALLITSEVA\_SÄÄ

Atmospheric pressure was excluded because while lower atmospheric pressure can be linked to less stable weather condition, its direct influence on driving is minimal. Additionally, this attribute was only retrievable from a handful of weather stations.
% 19	ILMANPAINE

Ice cover frequencies were also excluded as not relevant enough. While the frequency of ice can tell a lot about the qualities of the ice on a road surface (such as thickness), this value on its own tell us little about the driving conditions on the road. 
% 35	JÄÄTAAJUUS_1
% 36	JÄÄTAAJUUS_2
% 109	JÄÄTAAJUUS_3
% 119	JÄÄTAAJUUS_4
Similarly, the conductivity value of the road was ignored, as while this does aid in detecting water on the road surface, there are other attributes that provide more straightforward data on the exact topic that are easier to use. 
% 31	JOHTAVUUS_1
% 32	JOHTAVUUS_2
% 107	JOHTAVUUS_3
% 117	JOHTAVUUS_4

Some highly relevant attributes had to be excluded simply due to their availability. Such was the case with detailed snow depth, which differentiated between the depth of snow on road shoulders, on wheel ruts, as well as in between the ruts. This information would be very useful, as it helps detect the formation of heightened ruts due to the formation of snow and ice. % there's no word for polanne in english??
% 147	LUMENMITTAUS_A lumen paksuus reunaviivan kohdalla
% 148	LUMENMITTAUS_B lumen paksuus ajourassa
% 149	LUMENMITTAUS_C lumi ajourien välissä
% 150	LUMENMITTAUS_KA paksuuden keskiarvo

On the other hand some attributes were excluded because we were unable to definitively state their purpose or the data they gather. While we could form a variably educated guess on most of them we elected to rather rely on the attributes that are more clear. These unclear attributes include surface signal and fibre response, which quite likely have to do with monitoring the status of the station. 
The fibre response could also be related to detecting water or ice on the road, perhaps somewhat similarly to \cite{ruiz2011remote} where fibre optics were used in a system to detect water and ice on road surface.
% PINTASIGNAALI_1
% PINTASIGNAALI_2
% PINTASIGNAALI_3
% PINTASIGNAALI_4
% KUITUVASTE_PIENI_1
% KUITUVASTE_PIENI_2
% KUITUVASTE_PIENI_3
% KUITUVASTE_PIENI_4
% KUITUVASTE_SUURI_1
% KUITUVASTE_SUURI_2
% KUITUVASTE_SUURI_3
% KUITUVASTE_SUURI_4

\color{red}
\textbf{UNKNOWN}

% [TO-DO] Differences in sensor availability by station, also meta vs /data

The most common number of attributes per station (based on meta) is 129 with 424/533 stations in the country. Nine stations provide more attributes with a maximum of 147 attributes at a test station in Ranua.

According to FHWA, air temperature on its own has little affect on roads, traffic, or operations. 
% Liikenneturva: "Liukkaimmillaan tie on ilman lämpötilan ollessa lähellä nollaa" Also, autoja ei oo suunniteltu äärilämpöihin, kuten pohjantiellä näkee kun on -30C pakkasta.

Wind can cause visibility issues and lane obstructions, decrease the stability of a vehicle and increase travel speeds. Precipitation lowers visibility and road traction and can similarly cause lane obstructions. Fogs primarily affect visibility, while pavement temperature can cause damage to infrastructure(??). Rising water levels can cause lanes to be submerged, which increases the accident risk, among other things. % FHWA
% Liikenneturva: "Jos tiellä on paljon vettä, rengas saattaa nousta irti tiestä vesipatjan päälle. Vesiliirrossa autoa ei voi ohjata, koska renkaat eivät enää ole kiinni tiessä. Lumisohjossa auto voi joutua myös sohjoliirtoon, jopa herkemmin kuin sateella vesiliirtoon"
Overall, approximately 21\% of vehicular crashes in the US are weather related. The most significant factor in road safety appears to be rain and wetness of the road. 
% https://ops.fhwa.dot.gov/weather/q1_roadimpact.htm
% maybe get Finland data hear instead, sitäki on tarjolla. Tai vertailun vuoksi molemmat idk.
% ALSO: that statistic says nothing about how many % of rainy days have accidents, or snowy days etc., i would bet that it rains a lot more than it snows in the states.

\color{black}

\subsection{Weather Forecast}
On top of relaying data gathered by the road weather stations, the Digitraffic API also provides weather forecasts, that are specifically aimed for road traffic. The forecasts are not linked to specific weather stations, instead they are given to specific road sections. For each road section, four forecasts are provided, each of which further into the future from 2 to 12 hours. Additionally, the API provides an "observation", which could be considered a summary of the road weather station data. As we have left the time dimension without consideration, our focus was on this observation data, however the forecasts hold immense potential, as they would allow for more optimal route planning on longer distances without the need to recalculate the route along the way.

The content of both the observation and the forecast are similar. Both include data about daylight status, road and air temperatures, wind speed and direction, as well as overall conditions on the road. The condition can be defined as either normal, poor, or extremely poor. The condition definitions also include reasoning, for example if the overall condition is set as poor, this can be justified with a road surface condition, wind, precipitation, slipperiness, or visibility.
While this might seem that the condition information is sufficient for route planning and this data could render the more primitive weather station data obsolete, the weather forecast API has some some caveats. Most importantly, the threshold for determining the conditions as poor let alone very poor is rather high, meaning that cases when this happens are rare. This makes comparing routes somewhat difficult as for the most part, all routes have OK conditions. Additionally, some data is only available when it is used as justification for condition classification, as is the case with precipitation status for example. 
Then again it could be argued that the condition determined by the weather forecast observation provides a more reasonable classification of road conditions in the sense that minor issues are not blown out of proportion, instead the affect of truly troublesome conditions is emphasised. With this in mind, we attempted to combine the best of both worlds: to use the weather station data as described above, and additionally use the weather forecast observation as a sort of disaster indication index. If the condition reasoned in the weather forecast API is normal, the weight of the related road segments is zero. If the conditions are poor, the weight is 0.5 and if the conditions are extremely poor the weight is set at 1. However, the weather forecast data has one major caveat, that is, it can only be retrieved via a JSON query as it is not available through the MQTT WebSocket. As such this data was not present in our example cases. 


\subsection{Traffic Measurement Stations}
As stated are 520 traffic measurement in Finland, 15 of which have been temporarily removed, leaving us with 505 stations that are actively gathering data. The stations use a pair of induction loops to detect the passing vehicles, their lengths, and their speeds. The stations can also distinguish between directions and lanes used by the vehicles. 
%https://www.digitraffic.fi/tieliikenne/lam/

Traffic measurement stations produce fewer attributes than weather stations do, and they also come with additional documentation, leaving less room for misinterpretations. The meta introduces 103 traffic measurement attributes, numbered from 5016 to 100000. As with the weather attributes, many attributes can be considered sisters of one another, for example there are multiple attributes describing the travel speeds from the past 5 minutes on different lanes. The attributes can be categorised into three distinct groups: those detailing the speed of vehicles, those focused on the number of vehicles passing the station, and attributes describing both the dynamic and static characteristics of the station itself. While the the vehicle volume and speeds are monitored continuously, depending on the attribute, the corresponding values are not updated quite as often. Update intervals can range from three to five minutes up to an hour. There are also differences between stations: some stations boast a continuous real-time update rate, while most stations have an update interval of five minutes.

The Highway Capacity Manual (HCM) offers a guide for categorising roads based on the current Level of Service they can offer under the present circumstances. The LOS is defined as a scale from A to F with A being the best possible rating.
Multiple things affect the LOS category of a road, including vehicle volume and speeds \cite{hcm2010}.

\subsubsection{Vehicle Volume}
When the volume of vehicles on the road increases beyond the maximum capacity of the road, travel speeds start declining, congestion can form, and the risk of accidents increases. In the HCM, whether the vehicle volume exceeds the road capacity is used as a final threshold for determining whether the LOS of the road is classified as an E and and F \cite{hcm2010}. In route planning, one should strive for not only avoiding roads experiencing congestion, but also those where the risk of congestion is high. Therefore, instead of only concentrating on whether the volume exceeds the capacity, we focus more on how close the volume is to exceeding capacity.
The maximum capacities of each road segment are presented in the API, therefore we need not calculate the capacities ourselves.

The attributes come in two update types: the first one updates the data continuously according to the update rate of the station in question to reflect the situation within the past 3 or 5 minutes, while attributes of the other type are updated in regular 5 or 60 minute intervals. All values are extrapolated to one hour, if that is not already the time window used. Another divisive factor would be the level of specificity of the attribute: some attributes describe the volume on specific lane, others per direction, and one even overall.
There are huge differences in the availability of the attributes: while there are about a hundred stations that offer lane specific data about volumes, this is a clear minority. For the vast majority of the stations, the maximum level of detail is the volume per direction. Additionally, many roads in Finland only have two lanes, one in each direction, rendering lane specific details redundant. There is also really no sure way of attributing each of the fourteen possible attribute lanes to a physical lane based on the limited information that we have. Therefore we discarded all lane specific attributes. 
% OHITUKSET_3MIN_LIUKUVA_KAISTA1 - 14 -> discard
% OHITUKSET_5MIN_LIUKUVA_KAISTA1 - 14 -> discard
% OHITUKSET_5MIN_KIINTEA_KAISTA1 - 14 -> discard
We also discarded the attribute that did not differentiate between direction at all.
% OHITUKSET_5MIN_LIUKUVA_YHTEENSÄ -> discard

There are also multiple attributes that can be used to monitor the number of heavy goods vehicles on the road. While this data could be used to identify routes frequented by the vehicles, which in turn could be useful for determining personalised routes for users who particularly dislike driving among heavy goods vehicles. The data could also be experimented on for the tracking of exempt transports, that generally utilise large vehicles. However, this sort of analysis is beyond the scope of this paper, therefore the data pertaining to the heavy goods vehicles specifically is discarded at this point.

% OHITUKSET_60MIN_KIINTEA_SUUNTA1_LUOKAT245 --> discard
% OHITUKSET_60MIN_KIINTEA_SUUNTA1_LUOKKA2 --> discard
% OHITUKSET_60MIN_KIINTEA_SUUNTA1_LUOKKA4 --> discard
% OHITUKSET_60MIN_KIINTEA_SUUNTA1_LUOKKA5 --> discard
% OHITUKSET_60MIN_KIINTEA_SUUNTA2_LUOKAT245 --> discard
% OHITUKSET_60MIN_KIINTEA_SUUNTA2_LUOKKA2 --> discard
% OHITUKSET_60MIN_KIINTEA_SUUNTA2_LUOKKA4 --> discard
% OHITUKSET_60MIN_KIINTEA_SUUNTA2_LUOKKA5 --> discard

After discarding the lane specific attributes, attributes focused on heavy goods vehicles, and the attribute combining all vehicles passing the station, we are left with 10 direction specific attributes. While some stations might be located at crossroads or on bridges, they still only monitor the traffic on one specified continuous road, meaning that there are only ever two directions. 
In the traffic measurement data API, each direction has its own attributes. Half of these attributes report the number of vehicles passing the stations per hour, while the other half gives the percentage of how much the volume is of the maximum capacity of the road. Since the capacities differ greatly between roads, the flat volume does not communicate much about the conditions on the road, while the volume to capacity percentage is more telling as it takes into consideration the characteristics of each road, such as the number of lanes. By discarding all flat values,
% OHITUKSET_5MIN_LIUKUVA_SUUNTA1 --> discard
% OHITUKSET_5MIN_LIUKUVA_SUUNTA2 --> discard
% OHITUKSET_5MIN_KIINTEA_SUUNTA1 --> discard
% OHITUKSET_5MIN_KIINTEA_SUUNTA2 --> discard
% OHITUKSET_60MIN_KIINTEA_SUUNTA1 --> discard
% OHITUKSET_60MIN_KIINTEA_SUUNTA2 --> discard
we are left with six attributes, three per direction. The main difference between these attributes is their update cycle. The first one is updated continuously to reflect the conditions experienced in the past five minutes, while the other two are updated at regular intervals, either of five or 60 minutes. 
% OHITUKSET_5MIN_KIINTEA_SUUNTA1_MS1/2 --> discard
% OHITUKSET_60MIN_KIINTEA_SUUNTA1_MS1/2 --> discard
Because situations on the road can change rather quickly, we wanted to use the attribute that would be closest to real time as possible. Therefore we elected to utilise the continuous volume to capacity ratio as our attribute for vehicle volume.
% 5164	OHITUKSET_5MIN_LIUKUVA_SUUNTA1_MS1 => 0% -> 0, 100% -> 1.
% 5168	OHITUKSET_5MIN_LIUKUVA_SUUNTA2_MS2 => 0% -> 0, 100% -> 1.

For the sake of reliability, we could also calculate the ratio ourselves, using either the predefined maximum capacity or calculating the capacities our selves according to the instructions in the HCM, and the flat volume attributes. The predefined maximum capacity in each direction can be retrieved from a list of constants provided by the API. This list also contains The direction of the road in degrees, as well as free frow speeds (FFS).
% https://tie.digitraffic.fi/api/tms/v1/stations/sensor-constants
This should also be considered if the availability of the chosen attributes was low, however coincidentally, the availability of the continuous volume to capacity ratio attribute is exactly the same as that of the flat volume attribute. Therefore, availability should not be a concern with the chosen attribute.

As stated at the beginning of this section, for the purposes of route planning, we do not only wish to avoid routes that are already congested, but also those that have a high risk of becoming congested in the near future. The smaller the percentage is, the smaller this risk is, the higher the bigger the risk is. By this logic, when the value of the attribute is 0\%, the appropriate road segments will be given the weight of 0. Similarly, if the value is 100\% or more, the weight will be 1. Values in between are proportional to the percentages, so that e.g., with the volume reaching 50\% capacity, the weight of the segment will be 0.5.

The road directions are defined in the station meta based to the closest big city in either direction, making the interpretation of the directions easy for a human reader, but less so for a machine. The values of both "Direction1Municipality" and "Direction2Municipality" are given in the station meta as both name of the municipality and its official code assigned by the Digital and Population Data Services Agency. %https://dvv.fi/documents/16079645/20688161/Kommunkatalog+1.1.2024.pdf/de723369-d2ca-5c82-150d-df37cea3f759/Kommunkatalog+1.1.2024.pdf?version=1.7&t=1704194252458
In our case we only considered the trip from Oulu to Ylivieska, meaning that we could manually select the appropriate direction we wanted to consider for each station. In our case this was straightforward, as for the most part there was only one direction that could reasonably be considered (i.e., leaving Oulu, we would always drive in the direction away from it instead of towards it). In the future, a more robust way of determining the appropriate direction and choosing the attribute to consider should be devised. Additionally, considering the different values associated to driving the same road in different direction (i.e., considering the directions as separate vectors) could provide even more optimal routes to users.

\subsubsection{Vehicle Speed}
Tracking vehicle speeds is important as it provides the means for detecting obstructions on the road that might slow down the flow of traffic. These obstructions can be traffic jams, but might also include things like slow moving maintenance vehicles or traffic accidents. Slowing speeds can indicate issues even before the vehicles start to pack up, in other words before the volume starts increasing.

The Digitraffic attributes for vehicle speeds also contain those focused on specidic lanes as well as directions, just like volume attributes do. As with volume attributes, we disregard the lane specific speed attributes.
% LIUKUVA_NOPEUS_KAISTA_1 - 14 => discard
There are no attributes dedicated to heavy goods vehicles like there was with volume attributes. Instead, there are attributes dedicated to the slowest detected speeds. These could be useful for detecting abnormalities in the traffic flow, but for now we discard these attributes as their relevance to traffic conditions can be considered trivial.
% HITAIN_5MIN_LIUKUVA_SUUNTA1 => discard
% HITAIN_5MIN_LIUKUVA_SUUNTA2 => discard
% LIUKUVAN_NOPEUDEN_MINIMI_SUUNTA1 => discard
% LIUKUVAN_NOPEUDEN_MINIMI_SUUNTA2 => discard

The attributes 10 left are very similar to the volume attributes in that there are six attributes that only communicate the flat speed value measured within either a 5 or 60 minute window, and six attributes are updated in regular intervals while four are updated continuously. Eliminating the attributes providing flat speed values,
% KESKINOPEUS_5MIN_LIUKUVA_SUUNTA1 => discard
% KESKINOPEUS_5MIN_LIUKUVA_SUUNTA2 => discard
% KESKINOPEUS_60MIN_KIINTEA_SUUNTA1 => discard
% KESKINOPEUS_60MIN_KIINTEA_SUUNTA2 => discard
% KESKINOPEUS_5MIN_KIINTEA_SUUNTA1 => discard
% KESKINOPEUS_5MIN_KIINTEA_SUUNTA2 => discard
as well as those updated at regular intervals instead on continuously
% KESKINOPEUS_5MIN_KIINTEA_SUUNTA1_VVAPAAS1 => discard
% KESKINOPEUS_5MIN_KIINTEA_SUUNTA2_VVAPAAS2 => discard
left us with two attributes: the average speed in the past 5 minutes in either direction as a percentage of the free flow speed (FFS).
% KESKINOPEUS_5MIN_LIUKUVA_SUUNTA1_VVAPAAS1
% KESKINOPEUS_5MIN_LIUKUVA_SUUNTA2_VVAPAAS2
The directions associated with these attributes are the same as those concerning the vehicle volumes, therefore as we had already determined the directions to note for each station with the volume attributes, we could use these results for the speed attributes as well.

The FFSs of each station is defined both in the station meta, and the same list of constants that contained the capacity definitions. Each direction can have a different FFS. Additionally, on some roads the FFS is different depending on the time of the year. Digitraffic also provides classifications for the percentages to increase human readability. When the FFS is 0 to 10 percent of the FFS, it can be said that the traffic is stationary, at 10 to 25 percent the traffic is queuing, 25 to 75 the traffic is slow, 90 to 100 the traffic is fluent. If the percentage is larger than 100, that would mean the current speed is higher than the FFS \cite{lamDocumentation}. As a lower percentage signifies degraded traffic conditions, the smaller the attribute value, the higher the cost of the related road segment. Therefore, if the value of the average speed relative to the FFS is 0 \%, then the weight of that road segment is 1. If the relative speed is 100 \%, the weight is 0. Values is between are scaled so that 50\% is 0.5, 75\% is 0.25 etc.

\subsubsection{Station Characteristics}
As with the weather attributes, there are several attributes introduced in the meta, that should describe the state of the measurement station itself. None of these attributes are actually available through the data query itself, despite being included in the sensor meta. Some have corresponding attributes in the station meta data, and yet others have those in different meta queries, however linking these definitively is next to impossible. 
The station meta data does provide a collection status, purpose location information, collection intervals, among others,
% A_KERUUTILA?
% K_KERUUTILA?
% TILA?
% KERUULUOKKA?
as well as the municipalities in both directions of the road. It also lists the attributes that should be available at the station, and provides the FFSs in each direction. The direction of the road can be found in the list of constants discussed previously.
% NOPEUSSUOSITUS? 
% SUUNTA1
% SUUNTA2
% TIEN_SUUNTA
Alert levels, info screen texts texts and warning of the info screens are not present in any meta data, unless we consider them the equivalent of the attributes in the Variable Message Signs we will discuss shortly. 
% HALYTYSTASO
% INFOMERKKI_TEKSTI1
% INFOMERKKI_TEKSTI2
% INFOMERKKI_VAROITUS
Regardless, these attributes speak very little of the present conditions on the roads, therefore they were not considered for the weight vectors.

\subsection{Traffic Alerts}

Digitraffic relays traffic alerts related to four primary topics:  exempt transports, weight restrictions, maintenance, and traffic announcements which can include things like accidents.
The traffic announcements can be retrieved in either JSON or DATEX II format through the API. When received through the MQTT WebSocket API, the announcements are gzipped and need to be decompressed before they are readable.

\subsubsection{Exempt Transports}
Exempt transports require a specialised permit from the Centre for Economic Development, Transport and the Environment % ELY-keskus, lack of oxford comma in the official name ;P
due to their size or mass. These transports can hinder the flow of the rest of the traffic significantly, as they can require temporarily closing down intersections or parts of the road. The Digitraffic API provides some information about the exempt transports. This information includes the origin and destination municipalities, the dimensions exceeding the authorised limits of transport, the size of the entouerage, start and end times, as well as road legs and affect on other traffic. However, the issue with utilising this information is that this data is made first and foremost to be human readable. The level of detail is low which makes tracking these transports very challenging. As an illustrative real life example, an exempt transport 47 metres long and 7 metres high is travelling from Raahe to Oulu. From the API we know that this transport will cause the other traffic on the roads to be stopped at times, but our knowledge of the procession is limited. We only know that the transport should leave Raahe at 9:00, be in Oulu at 10:00, and the first road leg from Raahe to Liminka along road 8 should be done by 10:00. The last three road legs are also listed but no times can be estimated yet. The final road leg has no end point, therefore we have no idea how far along this road the exempt transport might travel. Additionally, the start and end points are only given as the names of municipalities. The only coordinates we have are those of the borders of these municipalities.

Avoiding all of these roads to avoid the exempt transport is impossible. Even only avoiding the next or current road leg is questionable at best. Depending on the transport travelling along the road, in a different or even the same direction can be completely unproblematic, as it is only the intersections onto the road that are affected. As the exempt transport completes road legs, the data is updated, therefore it is know which road leg will next be affected, if it is affected at all. This would also depend on the characteristics of road and it sections. As we have no way of knowing where exactly the transport is presently, at this time we cannot benefit from this data.

\subsubsection{Weight Restrictions}
As the name suggests, this category of alerts is concerned with restrictions on the weights of the vehicles travelling on the road. These alerts usually are concerned with temporary restrictions, and the data can include start and end dates to the restrictions. Unlike with exempt transports, the coordinates are given, and the affected road segments are described in detail. However, at this point we focused on passenger cars, which are most often not affected by these restrictions.
% these are only available through MQTT when they are pubished. For later use, they would either need to be saved to the routing server/cloud /whatever, or JSON queries need to be made when the route is calculated. Such is the case with all others too, but these can be months old.
\subsubsection{Road Work}
The road work API is used to provide information about current and upcoming road work operations. The information consists of location details and the work phase descriptions. The descriptions can include work times, start and end times, working hours, work types, as well as descriptions of the disturbance caused on traffic. For the purposes of route planning, this is perhaps the most important piece of information. This description includes things like the type of restriction imposed on traffic (closed lane, lowered speed limit, detours, etc.), whether the restrictions can be lifted, and severity of the disturbance (Low, High, Highest). 

In route planning, the current road work needs to be retrieved through the JSON API as the road works are only published through the WebSocket when they are new or updated. Additionally, many road work alerts contain information about road work that has been planned out into the future. This means that utilising the road work data requires more processing than for example weather data which is always current, as we need to distinguish between road work scheduled into the future, and the work currently underway. A small hindrance in the use of this data is that the data is clearly made to be very human readable with less consideration for machine readability. This is especially apparent with the free input comments and road work type descriptions, which appear to be manually written, based on variations in capitalisation, use of near synonyms, and mentions of specific roads or buildings within the description. This is mainly the case with road work where the type of work has been described as "other", which coincidentally appears to be the type of a third of all road work in September. 

Different types of road work would generally warrant different types of mitigation procedures for route planning, however as the type of road work can be almost anything thanks to the use of free form typing, this is not possible. Therefore our focus was on the severity of the disturbance, and weights to vectors representing the affected road segments will be allocated according to it. If there are no instances of road work affecting the segment, the weight is defined as 0. If the severity is defined as low, the weight is 0.33, if High the weight is 0.66 and finally, should the severity reach the rating of "highest", the cost is set at 1. 

As road work rarely comes on suddenly, it is likely that any affect the work has on the flow of traffic is also visible in the traffic measurement data throughout the duration of the work, depending on how far away from the road work site the nearest measurement station is located. The traffic measurement data also helps monitor the effects of road work on alternate routes, together enabling even more optimal route planning for the user.

\subsubsection{Traffic Announcements}
Traffic announcements are arguably the most relevant category of the four, these types of alerts provide information about events that have an immediate affect on traffic. Accidents are one of the most common topics of announcements provided in this category. Other topics include vehicles broken down on roads, animals on the road, large fires that affect traffic, or disturbances to ferry schedules and more. As there is no definitive list of all of the possible types of alerts, as there is not list for all types of road work, we could not device situation specific procedures for route planning. To add a layer of complexity, alerts come in six, set types: general, retracted, unconfirmed observation, ended, and the accident specific preliminary accident report and accident reports. 
We focused our attention on the handling of accidents due to the aforementioned lack of definitive list of topics. Typically, once an accident occurs, the first alert will be a preliminary accident report, which can be followed by an accident report or a general alert if the situation changes, or more details have become available. Once the accident has been cleared, an "all clear" is released. However, sometimes the only alert that gets released about an accident is the preliminary report. In such situations it can be difficult to know when the route is sensible to travel again, as there is very limited information available about the scale or affect of the accident. From their own web UI, Fintraffic removes preliminary accident reports without further details after about 30 minutes.
As there is no guarantee of detailed information, we assumed that all accidents are detrimental enough to the traffic flow that the road should be avoided. Therefore, any road segment with an accident is given the weight of 1, if the road segment has no accident, the weight is set to 0. A segment would be considered to having an accident if a) a preliminary accident report was published in the past 30 minutes or b) if an accident report of general announcement about an accident has been released with no announcement of the situation being over.

\subsection{Variable Message Signs}
As stated in the section \ref{relwo_VMS}, variable message signs are programmable road signs that can be set to display situation specific messages. In Finland, these signs come in three flavours: speed limits, information, and warnings. Information can be related to current weather (road temperature, air temperature, wind speed), delays in expected travel speeds, tunnel, road or lane being closed down, road maintenance ahead, poor driving conditions, missing road markings, etc. Warnings can be caused by e.g., road work, slippery roads, congestion, cross wind, uneven roads, loose gravel, dangerous road shoulders, ski tracks, or animals on the road. 
Much of the information available from the variable message signs is also available through other topics. Weather data, for example, has its own dedicated topic, which also provides info about driving conditions, road slipperiness. Congestion data is directly available from the traffic measurement topic. Closed roads, lanes, tunnels, bridges, animals on the road, and road maintenance are also communicated via traffic alerts. This would leave us with missing road markings, explicit delays in travel speeds, road surface warnings (unevenness, loose gravel, road shoulders), and ski tracks. While wind direction is provided in the weather topic, crosswinds are not explicitly identified.

The main issue with the use of variable message signs for the purposes of route planning however is their geographical disparity. The signs are heavily concentrated around the biggest cities and roads, mostly in Southern Finland (for comparison, in all of Lapland there are two signs, one in Pahtonen near Muonio and another in Kilpisjärvi while on Kehä III road in Helsinki alone there are 13 signs). The primary use case for VMS data would be for supplementing speed limit data of road segments with live data, which could be especially valuable for preference considerations in cases where speed limit or travel time is of utmost importance to drivers. Presence of warnings could be used for weighting roads but again due to the geographical distribution of the displays, this makes little sense as the few roads with signs would inevitably be rated more expensive as they are the only ones with available data. Therefore for now, the VMS data will not be used for route planning.

\subsection{Maintenance}
The maintenance API is focused on tracking maintenance vehicles completing various types of tasks on the road network. The API returns the task type and the path travelled by the vehicles, along with timestamps from up to 24 hours to the present moment. The API does not provide any planned events or paths and as such does not allow for predictive measures. The maintenance API meta introduces 38 different types of maintenance tasks. These tasks include things like cleaning, filling pot holes, salting and ploughing to name a few. Some maintenance types have a more profound effect on traffic than others, however quantifying this effect based on the little information available is next to impossible. The mere presence of maintenance does not necessarily affect the flow of traffic too much, but depending on the road geometry, speed limit, location, etc. the effect can be dramatic as well. For example, roadside mowing can done with a machine (that can be a normal tractor or something else) that moves slowly along the road. Depending on the speed limit, the difference can be huge or barely there, naturally a bigger difference will cause a bigger effect on other traffic on the road. Additionally, depending on the road geometry overtaking the mowing machine can be easy, which would lead to a smaller effect, or harder if the road is more narrow or winding, leading to a bigger effect. 

Due to this, as well as the fact that we only know where the maintenance vehicle has been, not where it is going, at this point we could not take this data into consideration. However, there is a lot of potential with the maintenance tracking for more optimal route recommendations, as it would allow us to track which roads have been ploughed and/or salted in the winter, leading to safer travels by preferring those roads, or tracking paving work to avoid any work sites or overly smooth, fresh pavement with no road markings. Additionally, some drivers might want to avoid the same maintenance tasks that others do not mind or might even prefer, for example in winter, some individuals prefer to drive on freshly ploughed roads, as close to the ploughing vehicle as possible, while others prefer to keep their distance as snow ploughs can send rocks flying into windows and obscure visibility in their surroundings. All this to say, that deciding on a definitive "good-bad" classification for maintenance tasks is difficult to say the least as it differs based on multiple variables. Additionally, for our purposes, any disruptive maintenance should be reported via traffic alerts, and as such, excluding the maintenance tracking from our consideration for route planning at this point should not affect the optimality of the route too much.


==> relwo-old.tex <==
\section{Related Work} 


To realise more optimal route planning in an ever changing environment, various types of real-world data need to be acquired and used. Fortunately, many modern road networks are already equipped with different types of technology to monitor the situation on the roads. This equipment can entail cameras, weather stations, various types of traffic measurement systems including inductive loop detectors, and road weather stations. Accident detection and maintenance tracking are equally important factors in ensuring safe travels for road users, as are variable message signs and other ways of alerting the public of tumultuous conditions. % [to-do] should i have references for all of these maybe?

Many applications already exist that utilise the real-time road data. Even the same data can be used for vastly different purposes. In the next sections we will go over some example uses of camera footage, as well as weather, weather forecast, and traffic measurement data, accident data and alerts, maintenance tracking data, and finally, the use of variable signs.

\subsection{Cameras} \label{relwo_cameras}
CCTV camera footage can be used for 
number plate recognition \cite{buch2011visionreview}, which can further be used to determine the volume and average speed of vehicles to assess the current traffic conditions \cite{zou2021cameratomap}. Vehicle counting in general is one of the most common uses of CCTV cameras on roads \cite{buch2011visionreview}. 
It is also possible to calculate travel times based on camera footage from intersections \cite{shao2020estimation}. Additionally, cameras aid in detecting incidents \cite{buch2011visionreview}, such as traffic accidents or violations \cite{anyang2016},
or congestion and traffic jams \cite{chakraborty2018traffic, kurniawan2018traffic}.
Recognising congested roads is important as it enables route planning around them. Additionally, detecting accidents via cameras makes it possible to alert emergency personnel and potentially save lives. This is an especially valuable application for scarcely trafficked roads \cite{ghosh2019accidentcamera}.
Weather conditions can also have a profound impact on roads. Images from road weather cameras can be used to determine the condition of the road and therefore whether there is need for dispatching maintenance, such as snowplowing and de-icing \cite{jonsson2011classification, grabis2022maintenance, anyang2016}.

Most cameras on roads are stationary, which introduces certain shortcomings. For example, hey can have limited visibility in certain weather conditions. To battle this, some works such as Chen et al. \cite{chen2022gocomfort} propose utilising autonomous vehicles, which possess mobile cameras that can reach areas beyond the line of sight of stationary ones. In their work, Chen et al. utilised the vehicle mounted cameras to capture images of potholes, which were then to be sent to a cloud centre for analysis and to be use in the creation of a high-definition map of the potholes in the road network. Such a map can then be used in optimising route planning for passenger comfort.

\subsection{Weather}
Considering weather conditions is important for route planning, because heavy rain or snow can reduce road capacity up to 17\% or 27\% respectively, in addition to reducing travel speeds. Rain can lower road capacity by 1\%-17\%, and speed by 1\%-7\%, depending on the intensity of the rain. Similarly, snow reduces capacity by 3\%-27\% and speeds by 3\%-15\%. \cite{agarwal2005weatherimpact}. Additionally, certain road weather conditions are linked to significantly increased accident risks \cite{malin2019accident}. It is no surprise that historic weather data together with accident records have been used in creating road risk indices for assessing the safety of road segments \cite{li2015roadrisk}. % [to-do] tähän joku kuolematilasto kuin monta autoilijaa sää tappaa?

Knowing the current condition of the road is also important for planning out and dispatching maintenance operations (appropriate use of which is invaluable especially during the winter). Air and surface temperature, humidity, dew point, precipitation and wind speed and direction can be used in determining whether a road is dry, wet, covered in snow, ice, or if it is snowy with tracks on it \cite{jonsson2011classification}. Based on data from road weather stations and predefined formal rules, it is possible to automate decision making regarding maintenance operations \cite{jokste2022latviamaintenance}. Being aware of the conditions on the road is equally valuable for route planning, as it makes it possible to avoid roads that are covered in a thick blanket of snow, or that are especially slippery or slushy. Furthermore, weather data has been used to predict the behaviour of other travellers. For example, current weather data has been considered as an explanatory factor for predicting traffic flow \cite{essien2021twitterweather} % temp. & precip.; traffic flow in this case means veh/h 
and travel speeds on roads \cite{kinoshita2017weather}. % temperature, snowfall, snow depth and precipitation 
Accurate predictions of traffic allow for more purposeful and informed decision making in route planning, as it enables avoiding congestion for example.

The specific type of weather data used differs vastly between applications. Some works have used only a few attributes while others have used multiple. For example, Ye et al. \cite{ye2024temperature} only used temperature values from the OpenWeather API and route planning by Google Maps to enable travellers to select more comfortable routes, while Jonsson et al. \cite{jonsson2011classification} used air and surface temperature, humidity, dew point, precipitation and wind speed and wind direction together with images from road weather cameras to determine the current weather conditions on the road. 

\subsection{Weather Forecasts}
%idk if it makes any sense to separate weather and weather forecasting, since forecasts are most often derived from current weather, but since digitraffic distiguishes between the two & they are different topics, for now let's.
While tracking the current conditions on the roads is invaluable, sometimes knowing the present state is not enough. If the route is only calculated based on the conditions prevalent at the beginning of the trip, towards the end of a long trip the conditions may have changed significantly. In such cases using weather forecasts instead of current weather can provide travellers with more appropriate route guidance throughout their trip. Using the predicted precipitation, wind, and surface temperature to estimate travel times of road segments as was done by Litzinger et al \cite{litzinger2012weatherroute} could help plan out even more optimal routes, and also estimate overall travel times with a higher accuracy.
Current road weather can be used as a basis for road weather forecasts to enable more localised weather forecasting. Road weather stations can be used to predict adverse weather conditions based on predetermined rules. This makes it possible to warn road users in advance of possible dangerous driving conditions \cite{tomas2016forecasting}. 

\subsection{Traffic Measurements}
Traffic measurement data can include vehicle speeds, traffic volume, and conditions. The data can be used for route planning, but also parking management and short-term traffic predictions. Various types of sensors are used to gather the data \cite{djahel2014communications}. One type of such sensors is loop detectors, which can be used to measure traffic speed and volume to determine prevailing traffic status \cite{anyang2016}. Loop detectors can be used for detecting traffic jams as well as accidents, or even vehicles travelling in the wrong direction, as they make it possible to calculate the speed of passing vehicles, as well as traffic volume \cite{jayasheelan2016tms}. 
Similarly, SCATS sensors have been used to gain access to traffic flow and vehicle speeds, which can then be used to create traffic predictions with the help of machine learning methods. The predictions can then be used as costs in route planning \cite{liebig2017predict}. Sensors can also be mobile, for instance deployed on taxis \cite{anyang2016}. Should congestion be detected or predicted, vehicles on the roads can be rerouted to avoid it \cite{de2016icarus}.

The importance of monitoring the current traffic situation is highlighted in cases where the time is of the essence. Such situations can include route planning for emergency services, that require the fastest possible route and cannot afford to get stuck in congestion. Tracking average travel speeds of each road segment is one way of using traffic data to realise optimal route planning in such a case \cite{al2018accident}. Regular drivers can have varying preferences on whether they want the fastest route based on current traffic situation, or perhaps the one that is generally the fastest based on historical data. Travel times derived from sensors play an important role in determining these routes here as well \cite{jakimavieius2010vilnius}.

% S P A R S I T Y  considerations, liebig ainakin mainittee
\subsection{Traffic incidents}
Different types of traffic incidents such as car crashes can majorly limit the capacity of a road segment creating the need for alternative routes to avoid the affected areas \cite{Dunn2006}.
Road incident involving different types of vehicles can present very different needs for route planning. For example, accidents involving hazardous chemical transport can have a dramatic affect on roads beyond the one where the accident took place \cite{li2024chemicalemergency}.
Generally, there are two approaches to dealing with accidents. The first one is a pre-emptive one, which entails assessing the risk associated with each road segment based on historic data \cite{li2015roadrisk}, and using the risk as a cost for route planning \cite{liao2022accident}.
The second approach focuses on handling accidents as they happen. Accident detection plays a key role in this approach. CCTV cameras can be utilised in identifying incidents on roads, and other road users can also report them \cite{anyang2016}. Additional sensors on board vehicles themselves can also be utilised in detecting accidents, for example by detecting the deployment of airbags \cite{sherif2014real}, or via OBD2 \cite{de2015garuda}. Vehicles can then alert a control centre so that emergency personnel can be dispatched \cite{sherif2014real} or a system can alert other road users via VANET to avoid the affected areas, and provide them with new routes \cite{de2016icarus}.
The Traffic Message Channel (TMC) is another way of warning driver of incidents that can potentially affect their travels. It is aimed at providing road users with up-to-date information about any relevant events on the road \cite{davies1989TMCstandards}. TMC can also be used to relay alerts about oncoming adverse weather to users \cite{tomas2016forecasting}. Taking TMC alerts into account in route planning makes it possible to avoid areas affected by different kinds of disruptions even before congestion begins to form.

\subsection{Variable Message Signs} \label{relwo_VMS}
Yet another method of information sharing are dynamic message signs or variable message signs (VMS). They are one of the traditional ways of relaying information to road users \cite{dey2014survey}. VMS are signs that can be programmed to display different messages. They go by many other names as well, such as changeable message signs \cite{Dunn2006} and variable message panels \cite{medellin2016}. The signs can be either portable or permanently installed to a specific location \cite{Dunn2006}.

VMS can be used to display many types of information to road users. They can be used for warning about current congestion \cite{anyang2016, medellin2016, namyangju2016}, potentially disruptive weather conditions \cite{peeta2001real, tomas2016forecasting}, as well as accidents \cite{anyang2016, medellin2016, namyangju2016}. They can be used to alert drivers about roads that have been closed down due to maintenance \cite{anyang2016, medellin2016}, and to guide drivers through maintenance sites \cite{xu2018vms-workzoneguidance}, or onto alternative routes \cite{Dunn2006}. Information about car park availability can also be provided via VMS for drivers' convenience \cite{anyang2016, namyangju2016}. They can also be used to educate drivers \cite{medellin2016} for example by displaying facts about car crashes \cite{kassens2021dms}, with the hope of influencing them to drive more carefully.

\subsection{Maintenance Tracking}
% Idk if I suck at searching or if it's just not done, but I genuinely cannot find articles that would do anything else. Even that is kind of hard to find. All route planning with maintenance focuses on routing the maintenance vehicles themselves, not other vehicles around maintenanace.

Road maintenance can reduce road capacity and cause congestion \cite{Dunn2006}. Despite this, maintenance activities are often ignored in route planning (beyond mentions of potential causes for congestion to be avoided), as is evident by the limited literature on the subject.
Automatic vehicle location systems can be used to track the location of the maintenance vehicle as well as any relevant info on the maintenance that was conducted (time, type, etc.). This information can be used as input for further maintenance decision making and reporting \cite{grabis2022maintenance, kocianova2015maintenance}. Maintenance vehicles could also potentially be fitted with sensors to monitor road conditions. \cite{kocianova2015maintenance}.

Maintenance vehicles often travel at slower speeds compared to ordinary travellers, or they can cause other disruptions to the traffic flow which can cause major inconveniences to other road users. Therefore avoiding road segments with active maintenance operations can be advised.

==> traffic-attribute-table.tex <==
\begin{table}[]
    \centering
    \scriptsize
    \begin{tabular}{|p{4cm}|p{2cm}|c|} \hline
         \textbf{Data item} & \textbf{Value} & \textbf{Weight} \\ \hline 
         \multirow{2}{*}{Free flow speed} &  100 \% & 0.0  \\
    & 0 \% &  1.0  \\ \hline

    \multirow{2}{*}{Vehicles / capacity} &  0 \% & 0.0  \\
    & 100 \% &  1.0  \\ \hline
         
    \end{tabular}
    \caption{An overview of traffic related attributes. The values in between the extrema are scaled.}
    \label{tab:traffic-weights}
\end{table}

